Bayesian Inversion for Anisotropic Hydraulic Phase-Field Fracture

In this work, a Bayesian inversion framework for hydraulic phase-field transversely isotropic and orthotropy anisotropic fracture is proposed. Therein, three primary fields are pressure, displacements, and phase-field while direction-dependent responses are enforced (via penalty-like parameters). A new crack driving state function is introduced by avoiding the compressible part of anisotropic energy to be degraded. For the Bayesian inversion, we employ the delayed rejection adaptive Metropolis (DRAM) algorithm to identify the parameters. We adjust the algorithm to estimate parameters according to a hydraulic fracture observation, i.e., the maximum pressure. The focus is on uncertainties arising from different variables, including elasticity modulus, Biot's coefficient, Biot's modulus, dynamic fluid viscosity, and Griffith's energy release rate in the case of the isotropic hydraulic fracture while in the anisotropic setting, we identify additional penalty-like parameters. Several numerical examples are employed to substantiate our algorithmic developments.

==> V7-Elsevier copy/conclusion.tex <==
%=======================================================================
\sectpa[Section7]{Conclusion}
%=======================================================================
In this paper, we presented an efficient numerical technique for hydraulic phase-field modeling including transversely isotropic and orthotropy anisotropic fracture. Here, three specific model equations in the sense of pressure, displacement, and crack phase-field have been coupled. Here, direction-dependent responses due to the preferred fiber orientation in the proelasticity material are enforced via additional anisotropic energy density function for both mechanical and phase-field equations. Furthermore, a new consistent additive split for the bulk anisotropic energy density function is introduced. More precisely, the new crack driving state function for poroelastic material was proposed in the sense that the compression mode of anisotropic energy is avoided to be degraded. Accordingly, we explained a fully monotonic solution for pressure and displacement, then a staggered approach has been employed for the crack phase-field equation. 

We presented a probabilistic setting for hydraulic phase-field fracture. We adjusted the DRAM algorithm to determine various effective parameters in crack propagation and hydraulic fracture. To that end, we used pressure during the fluid injection as the reference observation and strive to estimate six variables, including Lam{\'e} constants, Biot's coefficient, Biot's modulus, dynamic fluid viscosity, and Griffith's energy release rate. The approach compared to usual MCMC techniques, e.g., Metropolis-Hastings, showed more efficiency due to the proposal adaptation and the delayed rejection; therefore,
 a more reliable posterior density was obtained.

Specifically, the last two examples concerned with transversely isotropic and orthotropic anisotropic proelastic materials which used to demonstrate the feasibility and capability of the proposed model. 
 The finding showed that pressure evolves in the direction of the preferred fiber orientation in all numerical examples. Additionally, the fracture profile is aligned with the highest strength direction of the poroelastic material, which validate the efficiency and robustness of the model.  Additionally, we observed less influence of the penalty-like parameters used in the anisotropic density crack function. In these cases, the uncertainty arising for additional penalty-like parameters took into account.



%=======================================================================
\subsection*{Acknowledgment}

The first and the last authors have been financially supported by the German Research Foundation, 
Priority Program 1748 (DFG SPP 1748) in the 
subproject \textit{Structure Preserving Adaptive Enriched Galerkin Methods for Pressure-Driven 3D Fracture Phase-Field Models} 
with the project No.~392587580.

%=======================================================================



==> conclusion.tex <==
%=======================================================================
\sectpa[Section7]{Conclusion}
%=======================================================================
In this paper, we presented an efficient numerical technique for hydraulic phase-field modeling including transversely isotropic and orthotropy anisotropic fracture. Here, three specific model equations in the sense of pressure, displacement, and crack phase-field have been coupled. Here, direction-dependent responses due to the preferred fiber orientation in the proelasticity material are enforced via additional anisotropic energy density function for both mechanical and phase-field equations. Furthermore, a new consistent additive split for the bulk anisotropic energy density function is introduced. More precisely, the new crack driving state function for poroelastic material was proposed in the sense that the compression mode of anisotropic energy is avoided to be degraded. Accordingly, we explained a fully monotonic solution for pressure and displacement, then a staggered approach has been employed for the crack phase-field equation. 

We presented a probabilistic setting for hydraulic phase-field fracture. We adjusted the DRAM algorithm to determine various effective parameters in crack propagation and hydraulic fracture. To that end, we used pressure during the fluid injection as the reference observation and strive to estimate six variables, including Lam{\'e} constants, Biot's coefficient, Biot's modulus, dynamic fluid viscosity, and Griffith's energy release rate. The approach compared to usual MCMC techniques, e.g., Metropolis-Hastings, showed more efficiency due to the proposal adaptation and the delayed rejection; therefore,
 a more reliable posterior density was obtained.

Specifically, the last two examples concerned with transversely isotropic and orthotropic anisotropic proelastic materials which used to demonstrate the feasibility and capability of the proposed model. 
 The finding showed that pressure evolves in the direction of the preferred fiber orientation in all numerical examples. Additionally, the fracture profile is aligned with the highest strength direction of the poroelastic material, which validate the efficiency and robustness of the model.  Additionally, we observed less influence of the penalty-like parameters used in the anisotropic density crack function. In these cases, the uncertainty arising for additional penalty-like parameters took into account.



%=======================================================================
\subsection*{Acknowledgment}

The first and the last authors have been financially supported by the German Research Foundation, 
Priority Program 1748 (DFG SPP 1748) in the 
subproject \textit{Structure Preserving Adaptive Enriched Galerkin Methods for Pressure-Driven 3D Fracture Phase-Field Models} 
with the project No.~392587580.

%=======================================================================


